The dynamic effect of mechanical losses of actuators on the equations of motion of legged robots

Industrial manipulators do not collapse under their own weight when powered off due to the friction in their joints. Although these mechanism are effective for stiff position control of pick-and-place, they are inappropriate for legged robots which must rapidly regulate compliant interactions with the environment. However, no metric exists to quantify the robot's perform degradation due to mechanical losses in the actuators. This letter provides a novel formulation which describes how the efficiency of individual actuators propagate to the equations of motion of the whole robot. We quantitatively demonstrate the intuitive fact that the apparent inertia of the robots increase in the presence of joint friction. We also reproduce the empirical result that robots which employ high gearing and low efficiency actuators can statically sustain more substantial external loads. We expect that the framework presented here will provide the foundations to design the next generation of legged robots which can effectively interact with the world.

==> ideas.tex <==
% CONTRIBUTION: Recently backward driving has got more attention in the literature. However a rigorous formulation of power analysis is not yet present in robot literature. I'll talk about how to treat efficiency to formulate a generalized equation of motion for multi-DOF robots.  


% The motivation of this paper is  what is the better way to address actuators' energetic losses  to analyze and design the system-level dynamics, while joint-level friction model is not. Although friction and efficiency of an actuator can be used interchangeably to address dissipative loss, the access to friction model and efficeincy are different. 



% MOTIVATION: For example, it is easy to fasten a bolt with a driver, but impossible to unscrew the bolt by pulling it. Looking into the industry, factories are equipped with manipulators using high reduction harmonic drives. In both cases, friction contributes to low or non-backdrivability. 

% MOTIVATION: it is hard to backdrive or forward drive becuase t5here are combination of friction and efficiency. 

% IDK:While there are several papers addressing the asymmetry of forward and backward-driving efficiency, there has not been a rigorous formulation. 



% The essence of this simplified setup is that the friction is proportional to the reaction force between the block and the wedge, enabling both constraint force, $\bM A\T \lambda $, and a friction, $\bm f_\mu (\lambda)$, to be combined as a single term, where $\lambda$ is Lagrange multiplier and $\bM A$ is a constraint jacobian. To generalize this process, \textit{Lagrange multiplier matrix } and \textit{Efficiency Null} are introduced. Secondly, it shows bidirectional efficiency reported in the literature[][], suggesting that the dynamics of forward and backward-driving are different. Lastly, the distortion of inertia due to kinematic constraint and mechanical efficiency is formalized as matrix multiplication.  

To verify these points, three cases are analyzed; \textit{ideal} case, \textit{frictional and back-driving} case, and \textit{frictional and forward-driving} case. The generalized coordinate of this two-degree-of-freedom system is $ \bm q = [x, u]\T$. Note that power delivery is considered to be forward-driving if the wedge pushes the block.


\subsection{Ideal Case}
If kinetic friction is not present, the constraint force between meshed bodies does not produce work along the constrained surface. Notice that the constrained surface, corresponding to a holonomic constraint, $\gamma$, can be minimally expressed with $x$ and null-space matrix, $\mathbf{K}$. 
\begin{IEEEeqnarray}{rCl}
    \bm r &=& \bM A \T \lambda \\
    d\bm x &=& \bM K d \bm {q} \\
    dW_{c} &=& \langle d\bm x, \bm r \rangle = d \bm q\T \bM K\T \bM A\T \lambda = 0
\end{IEEEeqnarray}
where the constraint, $\gamma $, the constraint Jacobian, $\bM A$, its null-space matrix, $\bM K$, and constraint force, $\bm r$, are 
\begin{IEEEeqnarray}{rCl}
    \gamma &=& -x+ u  \cos \alpha = 0 \\ [3pt]
    \bM A&=& \pdif{\gamma}{\bm q} = \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
            -1 & \cos \alpha
        \end{IEEEeqnarraybox*}\right]\\
    \bM K &=& \nul(\bM A) =  \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
                        1 & \tfrac{1}{\cos\alpha}
                    \end{IEEEeqnarraybox*}\right]\T 
\end{IEEEeqnarray}

Following [], the equation of motion is acquired by multiplying $\bM K\T$ to constrained dynamics, 
\begin{gather}
    \bM H \ddot{\bm q} -\bM A\T \lambda = \bm f  \\
    \bM K\T \bM H \bM K \ddot{x} = \bM K\T \bm f  \\
% \end{IEEEeqnarray}
% \begin{IEEEeqnarray}{rCl}
    \bM H = \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
                M & 0 \\ 0 & m
            \end{IEEEeqnarraybox*}\right], \;\;\;\;
    \bm f = \left[\begin{IEEEeqnarraybox*}[][c]{,c,}
                f_x \\ -f_u
            \end{IEEEeqnarraybox*}\right]        
\end{gather}

\subsection{Back-driving Case}
The block and wedge are pushed by $f_x$, and kinetic friction is present between the slope and the wedge. The kinetic friction, $\bm f_\mu$, at the constrained surface is proportional to the constraint force. The friction and constraint force are added and treated as a revised constraint force, $\tilde{\bm r}$. 
\begin{gather}
\tilde{\bm r} := \bM A\T \lambda_x + \bm f_{\mu }(\lambda_x) \\
\bM H\ddot{\bm q} - \tilde{\bm r} = \bm f_{\rm ext} 
\end{gather}


To clearly state the directionality of power delivery and to formulate more concisely, \textit{Lagrange multiplier matrix}, $\bM \Lambda $, and efficiency matrix, $\bM \Gamma$, are introduced, where $\eta$ is the mechanical efficiency of the transmission. The revised constraint force is expressed as matrix multiplication, 
\begin{IEEEeqnarray}{rCl}
    \tilde{\bm r} &=& \bM \Gamma^{-1} \bM A\T \lambda_x \\
              &=& \bM \Lambda \bM A\T
\end{IEEEeqnarray}
where
\begin{gather}
\bM \Lambda= \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
                    \lambda_x & 0 \\ 0 & \lambda_u
                \end{IEEEeqnarraybox*}\right], \;\;\;\; 
\bM \Gamma = \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
                    1 & 0 \\ 0 & \eta_{\rm b}^{-1}
                \end{IEEEeqnarraybox*}\right] 
\end{gather}
Notice that the back-driving mechanical efficiency is identical to the ratio of meshing forces, assuming the kinematic constraint is conserved. 
\begin{IEEEeqnarray}{rCl}
    \eta_{\rm b} = 1-\mu \tan\alpha = \frac{\lambda_u}{\lambda_x}
\end{IEEEeqnarray}

Multiplying the whole equation by $K\T \Gamma$ reduces the model to one-degree-of-freedom system and cancels the Lagrange multiplier matrix. In this procedure, \textit{efficiency null}, $e$, is introduced to generalize this concept in the following sections, 
\begin{IEEEeqnarray}{rCl}
e:=\bM{K\T \Gamma \Lambda A\T} = 0
\end{IEEEeqnarray}

The the lossy dynamics in $x$ is obtained by multiplying $\bM K\T \bM \Lambda$ both sides,  
\begin{gather} 
\bM{K\T \Gamma H K} \ddot{x} = \bM {K\T \Gamma} \bm f_{\rm ext}\\
\left(M + \frac{1}{\eta_{\rm b}}m\sec^2 \alpha \right) \ddot x =  f_{x} \label{eqn:exampleReducedEoM}
\end{gather}

The eqn. [\ref{eqn:exampleReducedEoM}] captures the nature of constrained lossy dynamics. First, the apparent inertia is inflated by the reciprocal of the mechanical efficiency, suggesting that the system feels heavier than what would an ideal system feel like. Second, the equation is analytic; Even though the friction model is simplistic, designers have analytical tool to compensate for the friction at the early design time. 


\subsection{Forward-Driving Case}
In this case, a force, $-f_u \hat{\bm u}$, is applied to the wedge, but the coordinate of interest is again $x$. The model of dynamics identical to eqn (17), but several terms and parameters are different as to the direction of power delivery. The forward-driving efficiency, $\eta_{\rm f}$, and the efficiency matrix, $\Gamma$, are different from that of back-ward driving case, given as
\begin{gather}
    \eta_{\rm f} = \frac{1}{1+\mu \tan\alpha }= \frac{\lambda_x}{\lambda_u}\\[3pt]
\bM \Gamma = \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
                    1 & 0 \\ 0 & \eta_{\rm f}
                \end{IEEEeqnarraybox*}\right] 
\end{gather}
The lossy dynamics of forward-driving case is calculated in the same manner,
\begin{IEEEeqnarray}{rCl}
    \left( M + \eta_{\rm b} m \sec^2\alpha \right)\ddot{x}=-\eta_{\rm b}f_u \sec \alpha = -\eta_{\rm b} \hat{f_x}
\end{IEEEeqnarray}
where $\hat{f_x}$ is the input force converted in $x$ coordinate frame. 

% ===========================================================================
% iThe derivation includes the concept of holonomic constraint, model reduction, reflected inertia, and mechanical efficiency. The model shown in Fig. [] is a rectilinear equivalent of a robotic arm being back-driving by external force. The body \(M\) and \(m\) represent for the structural inertia of a limb, and the rotational inertia of a rotor. This minimal model schematizes a general kinematic meshing with friction, by introducing a non-smooth slope. 

% The horizontal force pushes block \(M\), only to move horizontally, and the wedge \(m\) moves along the slope. Notice that gravity is not present, and contacts are maintained. The derivation of equation of motion consist of analysis on parts; model reduction with constraint, meshing force balance, and directionality power flow. 
% As there exist one kinematic constraint, the whole system can be minimally represented with coordinate \(x\).  Given generalized coordinate, \(q=[x, u]\T\), the constraint jacobian and its nullspace matrix are
\begin{IEEEeqnarray}{rCl}
    C &=& x-\scos_\alpha u = 0 \\ [3pt]
    A&=& \pdif{C}{q} = \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
            1 & -\scos_\alpha
        \end{IEEEeqnarraybox*}\right]\\
    K &=& \nul(A) =  \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
                        1 & {\sec_\alpha}
                    \end{IEEEeqnarraybox*}\right]\T
\end{IEEEeqnarray}
% where \(c_\alpha = \cos(\alpha)\), and $ sec_\alpha=\sec(\alpha) $. Assuming the constraint being conserved, the mechanical efficiency of the entire system, $\eta$, equals the ratio of the meshing forces between $M$, and $m$,
\begin{IEEEeqnarray}{rCl}
    \eta = 1-\mu \tan\alpha = \frac{\lambda_u}{\lambda_x}
\end{IEEEeqnarray}
% where $ \lambda_x $, and $ \lambda_u $ are net meshing forces along the direction of $x$ and $u$ acting on body $M$, and $m$. The mechanical power flows from $x$ to $u$. Notice that actual net reaction forces are $R_x$, and $R_u$, which are different from $\lambda$'s. Using the constraint jacobian and its nullspace matrix, acceleration and reaction forces can be represented as, 
\begin{IEEEeqnarray}{rCl}
    \ddot{q}&= &K\ddot{x} \\[4pt]
    R &=& \Gamma A\T
\end{IEEEeqnarray}

In the sense of duality, the mechanical power flow of the entire system should satisfy \textit{efficiency null form}, $E$. Note that $E$ is always zero except static condition, $dx=0$. 
\begin{IEEEeqnarray}{rCl}
    &&0=\eta \langle dx, R_x\rangle + \langle du, R_u\rangle = dq\T \Gamma R \\ [4pt]
    &\Rightarrow &0= dx\T \underbrace{K\T \Gamma \Lambda A\T}_{:=E} 
\end{IEEEeqnarray}

% To obtain the equation of motion, the efficiency null is utilized to cancel out the constraint force term of constraint dynamics. Since the meshing forces are not equivalent, the Lagrange multiplier is generalized to address the directionality of power flow. 
% \begin{IEEEeqnarray}{rCl}
%   \dif{ }{t}\pdif{L}{\dot{q}}-\pdif{L}{q}-\Gamma A\T m &=& f \\ [4pt]
%   H\ddot{q}+C-\Gamma A\T m &=& f 
% \end{IEEEeqnarray} % !!!!!!!!!!!!!!!!!!! REDUCE THE Line Distance!!!!!!!!!!!!!!!!!!!
% \begin{IEEEeqnarray}{rCl}
%   \Rightarrow &K\T \Gamma H K \ddot{x} + K\T \Gamma C = K\T \Gamma f
% \end{IEEEeqnarray}

% The inertia of eqn () includes the body mass of the brick, as well as the apparent, or reflected inertia, $m \sec^2 \alpha $, of the wedge. The reflected inertia feels heavier as the friction is addressed by the reciprocal of mechanical efficiency. In the following sections, this idea is expanded to general robotic systems with higher degrees of freedom. 
% \begin{IEEEeqnarray}{rCl}
%   \bar H(\eta) &=& \left[\begin{IEEEeqnarraybox*}[][c]{,c,}
%                         1 \\ \sec_\alpha 
%             \end{IEEEeqnarraybox*}\right]\T
%             \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
%                 1 & 0 \\ 0 & {\eta}^{-1} 
%             \end{IEEEeqnarraybox*}\right]
%             \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
%                 M & 0 \\ 0 & m
%             \end{IEEEeqnarraybox*}\right]
%             \left[\begin{IEEEeqnarraybox*}[][c]{,c,}
%                         1 \\ \sec_\alpha 
%             \end{IEEEeqnarraybox*}\right] \\ [5pt]
%         &=& M + \frac{1}{\eta}m \sec^2 \alpha
%             % \left[\begin{IEEEeqnarraybox*}[][c]{,c/c,}
%             %     \lambda_x & 0\\ 0 & \lambda_u
%             % \end{IEEEeqnarraybox*}\right]
% \end{IEEEeqnarray}
% ===================================================



\subsection{Redundant Rigid Body Model and Model Reduction} 
The effect of mechanical efficiency of transmission on a generFal floating-base robot is analyzed. The state space of this robot is\(n\)-dim space, which is the sum of 6 free DOF for floating base and \(m\) DoF for actuated links. Also, this robot is equipped with \(m\) motors. In order to account for \(m\) rotors in the motors, we augment the DoF to \(n+m\), as if the rotors are freely dangling to the system. Then, the system DOF is reduced to \(n=(n+m)-m\) with \(m\) independent constraints that represent kinematic coupling or meshing between a rotor and a structural body. 

The redundant state is defined as $s\ns=\ns\rowvector{q_b\T, \,q\T\!, \phi\T }\T $ and minimum state is $y  = \rowvector{q_b\T, \,q\T}\T \ns\in\ns\R^n$, where $q_b \ns \in \ns \R^6$,  and $q, \, \phi \ns \in \ns \R^m $. The kinematic constraint, $C$, is holonomic, and its constraint jacobian, $A$, and the constraint null space, $K$, are
\begin{IEEEeqnarray}{rCl}
    C &=& q - D G\phi =0 \in \R^m\\[4pt]
    A &=& \tpdif{C}{s}=  \bmat{\;\; 0_{m\times6} & 1_{m}& -DG \;\;} \in \R^{m\times(n+m)}\\[4pt]
    K &=& \bmat{\;\;1_6 &0 \\ \;\;0 & 1_m \\ \;\;0 & -(DG)^{-1}} \in \R^{(n+m)\times n}
\end{IEEEeqnarray}

The efficiency null form (\ref{eqn:effNull}) is generalized, in order to account for the individual mechanical efficiency of transmission. For every coupling between $\phi_j $ and $q_j$ for $j=1\cdots m $, the efficiency null, $E_j=0$ is zero, as well as the column vector form. 
\begin{IEEEeqnarray}{rCl}
    0 & = & \bmat{0_6, E_1, E_2, \cdots, E_m}\T \\[4pt]
    &=& \dot{s}\;\Gamma M = (K\dot{y})\T \Gamma \Lambda A\T m  
\end{IEEEeqnarray}

The generalized efficiency matrix, $\Gamma$, and the generalized Lagrangian multiplier matrix, $\Lambda$ are defined as, 

\begin{IEEEeqnarray}{rCl}
    \Gamma &=& \bmat{1_6 & 0 & 0 \\ 0 & 1_m & 0 \\ 0 & 0 & \diag(\delta_j)} \\[4pt]
    \delta_j &=& \begin{cases} \eta_F^j & \text{forward-driving} \\1/\eta_B^j & \text{back-driving} \end{cases} \\[4pt]
    \Lambda &=& \diag({1_6, \lambda_1^i, \lambda_2^i, \cdots, \lambda_m^i, \lambda_1^o, \cdots, \lambda_m^o})
    %Λ_io=diag(1_m,λ_1^out,…,λ_c^out,λ_c^in,…,λ_c^in) 
\end{IEEEeqnarray}
 
Figure (energy flow between gears, three kinematic trees)

If all eta = 1, then eqn(eta) = eqn0

Back-driving/Forward Driving Cases

Show what happens to reflected inertia if eta -> 0

\subsection{Relaxation for Theoretical Consistency}
A forced conversion from Non-symmetric Inertia Matrix to Symmetric Matrix

Error analysis





% ====== PAR0. Dissipative Force and Real-model gap, possibly valuing efficiency more. 
% actuator efficiecny plays a major role in the system level dynamics of a robot. for instance.. conven high ratio low eff HD makes it statue dangerious, key factor are .... high friction efficiency.... they don't fall with gravity.. what's causing low eff, and large friction
% Expectation for the robots to be the first responders and master crafters has put actuators and mechanisms into challenges. As these hardware evolves, it is important to recognize its inevitable limitations and their influence on the entire system, in order to fully exploit it as hardware components. The friction inherent to machines and the consequent degradation of mechanical properties have been impairing dynamic and precise motion control. While industrial transmission or gearbox is conventionally powerful enough to marginalize internal frictions, but in case of more demanding systems such as locomotive robots, they respond slowly and inaccurately to the control command with the presence of the friction in transmissions. For future robots, designers may take mechanical efficiency, as a characteristic behavior of friction, into design consideration to compensate for above friction-induced degradation. In this regard, we present a framework to analyze the system performance with individual actuator efficiencies.
% Robotic first responders are expected to perform physically demanding labor which pushes the limits of their actuators. And despite the remarkable advances in actuator technology, their performance is still inevitably limited the mechanical efficiency which is governed by energetic losses. For instance, the inherent friction of the transmission degrades the robots' capability of precisely control its motion and to compliantly interact with the environment. Although compact, the low efficiency gearboxes, such as harmonic drives, have been widely utilized for stiff position control, they are not appropriate for legged robot which must regulate the contact  with the environment. To be able to precisely regulate 
% The key property that determines the precise regulation of contact forces is the actuator efficiency. 

% systems such as locomotive robots, they respond slowly and inaccurately to control command with the presence of the internal friction. 

% of mechanical properties impairs dynamic and accurate motion control as a whole robot. While industrial transmissions or gearboxes are conventionally powerful enough to marginalize internal frictions, more demanding systems such as locomotive robots, they respond slowly and inaccurately to control command with the presence of the internal friction. 
% example > non-backdriv > why efficiency/friction > nonlinear > hard to control > gap


% third possibility available at design time, which is to estimate the degradation of system performance originating from the individual actuator efficiencies.

% And thus, the dissipative forces in the transmission evidences the gap between real robot and their simulated dynamic model. Therefore it is a good idea to minimize the difference. 
% The friction in a transmission negatively affect dynamics of a system. For example, the wheel of a bicycle feels a lot heavier even if brakes are partially engaged. 
% Come up with an example that explains how friction affects mass.force.impedance... And it really affects it cite papers about it. 

% The motivation of this paper is to answer a following example. Given a manipulator design problem using conventional low-efficiency harmonic drives as joint transmissions, how can a designer predict the system behavior? That is to say, how much is it different from having a frictionless transmission? 


% ====== Whats the implication of this pmaper and safely interact with surroundings. From navigating rugged terrain to safely lifting  


% Since friction contributes to lower mechanical efficiency, The point of this paper is that the actuators' dissipative loss can be treated differently according to researchers' task; to control, or to design a robot. 
% the higher friction results in low mechanical efficiency. 

% The goal of this letter is to study the effect of joint level efficiency to the system level dynamic behavior. To illustrate this, an example - given two different actuators which one goes to where..

% Not to mention the nonlinearity / stochastic of friction, there exists uncharted behavior such as non-backdrivability of high reduction ratio harmonic drives. Although it is incomplete, there are two major approaches to dealing with dissipative loss; using intricate friction or damping models or identifying their mingled effect as mechanical efficiency. While latter approach has not been drawing attention in the robot literature, this paper gives light on the advantage of it; the mechanical efficiency captures peculiar aspects of transmission. For example, the above non-backdrivability can be addressed by setting the backdriving efficiency as zero, while model-based approach needs more work. 

% ====== PAR1. Detrimental effects of friction - I need to really explain what these effects, examples and connect
% The dissipative loss is detrimental to robotic transmissions, since it contributes to high mechanical impedance, low or even non-backdrivability and asymmetric dynamics(lead screw). In general, these traits impede robots from achieving dynamic motion or safe interaction with the world. Talk about how these affect dynamics with references..
% does more harm than simply degrading torque and power delivery; it contributes to . These undesirable traits generally impede a robot from dynamic motion and safe interaction \cite{safeSami}. 

% ====== PAR2. What friction means to designers
% The energetic losses of the transmissions at joint level complicate the design of the robot at the system level. This difficulty arises from the lack of a design criteria which describes how the efficiencies of individual actuators propagate to the dynamic behavior of the whole system. The fundamental issue caused by this challenge is that the designer cannot predict the system performance degradation due to friction \textit{a priori}. One must first build a robot and next experimentally estimate a model for the losses which is specific to that particular mechanism. (). A second issue caused by the lack of a metric which maps the actuator losses to the system level is that designers may not a have a unique optimal choice for candidate transmissions. For instance, if you would have to choose between 

% The lack of a metric which maps the actuator losses to the system level prevents designers from selecting between candidate transmissions when task-space backdrivabiltiy and low reflected inertia is a system requirement. In one hand, choiceMotorReducer, on the other hand, wensing. However, the effect of individual loss of transmission on a whole robotic system still remains unstudied. (CONTRIBUTION: This paper fills the gap)

% influence of internal loss on the whole system, two problems arise in the early stage of design. First, design process becomes unidirectional that a designer should develop a physical model and then run a simulation to witness the consequences of internal friction. This is problematic as the result is often numerical, not analytic, and requiring time and experience for a designer to improve the design. Secondly, the optimal choice of the type of actuator and drivetrain remains unclear. In this regard, Giberti provides a guideline for the choice of a paring of actuator and reducer,  considering joint level efficiency \cite{choiceMotorReducer}. Wensing investigates how joint-level inertia-dependent backdrivability aggravates the the impact mitigation of a whole system \cite{impactMitigation}. However, the effect of individual loss of transmission on a whole robotic system still remains unstudied.
% whose actuators are pushed to the envelope

% ====== PAR3. Fundamental Question
% The point of this paper is to investigate how joint level mechanical efficiency affects the dynamics of the whole system. 
% Specifically, this paper considers following problem. Given a 2-degree of freedom(DoF) serial legged robot and two different actuators that have the same torque capability, but different gearing ratio and mechanical efficiency, which actuator should be attached to the hip or the knee joint, so as to minimize task-space inertia felt at the ground contact? That is, how do we leverage the change in torque delivery, reflected inertia, mechanical impedance, and backdrivability which are all brought by joint-level internal friction, from entire system's perspective?



\section{Related Works}
% GEARING EFFICIENCY - velocity/load dependence, efficiency in the inertia term, recent bidirectional efficiency, how SEA is free of this issue?, yada-asymmetry in torque delivery, friction compensation techniques, joint friction, transmission characteristic(one of reviews), recent paper on high efficiency gears, velocity matching and contact

% There are multiplitude of influence a transmission brings to a dynamic system. Both ideal and lossy cases have increased reflected inertia and mechanical impedance. This tendency is even stronger for lossy case where dissipative forces such as friction or damping exists. Moreover, the dissipatice force is responsible for asymmetric behaviour; having different mechanical efficiency according to the direction of power delivery. In this regard, \cite{choiceMotorReducer} propose guidelines for the choice of motor-reducer pair,  \cite{DirectionalEff} [Hamon, Wu] verifies directional differences, and \cite{BilateralEff} shows that backward-driving efficiency is always smaller than the other. Yada enlightens that both force delivery and line of action are distorted by the friction \cite{Yada} 

% The internal friction also debase the backdrivability, even rendering a system to be non-backdrivable \cite{WAMTownsend}, \cite{BilateralEff}. 

% friction but the rate of increase for  

% and damping in the lossy transmission worsens 


% FRICTION IDENTIFICATION AND COMPENSATION the - lot obut the rate of increase for  

% f them
% % Fast forward dynamics simulation of robot manipulators with highly frictional gears
% BACKDRIVABILITY - inertia/friction depen -\cite{WAMTownsend}, hydraulic, LIMBS1 and LIMBS2, Reduction of reflected inertia is required for contacts - sami hadd

% DESIGN METRICS - handbook of robotics
% Model-Based Hydraulic Impedance Control for Dynamic Robots
% Disturbance-Observer-Based Compliance Control of Electro-Hydraulic Actuators With Backdrivability
% In [9], an effective model-based impedance controller was
% developed for a legged robot with EHSSs by introducing an
% inner-loop force/torque controller

% RIGID BODY SYSTEM - featherstone, long-hold paradox - unbounded friction and measure theory, which is not the focus of this paper, 

% The mechanical efficiency has been appearing in the inertia term in the gear literature \cite{BilateralEff} \cite{DirectionalEff}.



